Quantum State Preparation Circuit Optimization Exploiting Don't Cares

Quantum state preparation initializes the quantum registers and is essential for running quantum algorithms. Designing state preparation circuits that entangle qubits efficiently with fewer two-qubit gates enhances accuracy and alleviates coupling constraints on devices. Existing methods synthesize an initial circuit and leverage compilers to reduce the circuit's gate count while preserving the unitary equivalency. In this study, we identify numerous conditions within the quantum circuit where breaking local unitary equivalences does not alter the overall outcome of the state preparation (i.e., don't cares). We introduce a peephole optimization algorithm that identifies such unitaries for replacement in the original circuit. Exploiting these don't care conditions, our algorithm achieves a 36% reduction in the number of two-qubit gates compared to prior methods.

==> figure/fidelity-comparison.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=.6\linewidth]{img/resynthesis_avg_fidelity.pdf}
    \caption{Fidelity comparison}\label{fig:results-scalability}
\end{figure}


==> figure/initial.tex <==
\begin{figure}[hbt]
\centering
\mbox{
\small
    \Qcircuit @C=.7em @R=.3em {
            && \mbox{$\ket{\psi_1}$} & \mbox{$\ket{\psi_2}$} &\mbox{$\ket{\psi_3}$} & \mbox{$\ket{\psi_4}$} & \mbox{$\ket{\psi_5}$} & \\
\lstick{q_0} & \gate{\parbox{0.6cm}{\centering \footnotesize $R_y$\\$\pi/2$}} \ar@{--}[]+<1.7em,1em>;[d]+<1.7em,-3em> & \ctrl{1} \ar@{--}[]+<1.7em,1em>;[d]+<1.7em,-3em> & \ctrl{1} \ar@{--}[]+<1.7em,1em>;[d]+<1.7em,-3em> & \qw \ar@{--}[]+<1.7em,1em>;[d]+<1.7em,-3em> & \qw \ar@{--}[]+<1.7em,1em>;[d]+<1.7em,-3em> & \qw \\
\lstick{q_1} & \qw & \gate{\parbox{0.6cm}{\centering \footnotesize $R_y$\\$\pi/2$}} & \ctrlo{1} & \gate{\parbox{0.6cm}{\centering \footnotesize $R_y$\\$\pi/2$}} & \ctrl{1} & \qw \\
\lstick{q_2} & \qw & \qw & \gate{\parbox{0.6cm}{\centering \footnotesize $R_y$\\$\pi$}} & \qw & \gate{\parbox{0.6cm}{\centering \footnotesize $R_y$\\$\pi/2$}} & \qw
    }
}
\caption{Initial circuit to prepare state $\ket{\psi}$.}\label{fig:initial}
\end{figure}

==> figure/resyn-optimized.tex <==
\begin{figure}[t]
\centering
\mbox{
\small
    \Qcircuit @C=.7em @R=1em {
         \lstick{q_1:} & \qw & \qw           & \ctrl{2}          & \qw           & \qw  & \qw           &  \qw \\ 
         \lstick{q_2:} & \qw & \qw           & \qw     & \qw       & \ctrl{1}     & \qw                 &  \qw \\
         \lstick{q_3:} & \qw & \ry{-\frac{\pi}{4}} & \targ        & \ry{\frac{\pi}{2}} & \targ     & \ry{-\frac{\pi}{4}} &  \qw
    }
}
\caption{Optimized subcircuit}\label{fig:exact-synthesis-mcry}
\end{figure}

==> table/results.tex <==
\newcommand{\highlight}[1]{{\cellcolor{yellow} \textbf{#1}}}

\begin{table*}[]
\renewcommand{\arraystretch}{0.8} % Default value: 1

\centering
\footnotesize
\begin{tabular}{c|c|cc|ccc|ccc|ccc|ccc|ccc}
\hline
 &
   &
   &
   &
  \multicolumn{3}{c}{Initial} &
  \multicolumn{3}{|c}{Qiskit} &
  \multicolumn{3}{|c}{PyZX} &
  \multicolumn{3}{|c}{A* search} &
  \multicolumn{3}{|c}{\highlight{DC-Resyn (ours)}} \\
\hline
 &
  Init &
  $n$ &
  $m$ &
  \#G2 &
  \#G &
  T &
  \#G2 &
  \#G &
  T &
  \#G2 &
  \#G &
  T &
  \#G2 &
  \#G &
  T &
  \#G2 &
  \#G &
  T \\
\hline
\multirow{3}{*}{W} &
  m- &
  3 &
  3 &
  4 &
  4 &
  0.002 &
  4 &
  13 &
  0.005 &
  4 &
  16 &
  0.004 &
  4 &
  3 &
  0.007 &
  4 &
  4 &
  0.001 \\
 &
  m- &
  6 &
  6 &
  13 &
  10 &
  0.015 &
  10 &
  52 &
  0.138 &
  19 &
  46 &
  0.012 &
  13 &
  9 &
  1.420 &
  13 &
  10 &
  0.003 \\
 &
  m- &
  9 &
  9 &
  22 &
  16 &
  0.125 &
  16 &
  88 &
  0.146 &
  34 &
  76 &
  1.065 &
  22 &
  15 &
  1.506 &
  22 &
  16 &
  0.007 \\
\hline
avg &
   &
   &
   &
  13 &
  10 &
  0.047 &
  \highlight{10} &
  51 &
  0.097 &
  19 &
  46 &
  0.360 &
  13 &
  9 &
  0.978 &
  13 &
  10 &
  0.003 \\
\hline
\multirow{5}{*}{$\ket{D_n^k}$} &
  m- &
  3 &
  3 &
  4 &
  4 &
  0.002 &
  4 &
  13 &
  0.004 &
  4 &
  16 &
  0.003 &
  4 &
  3 &
  0.009 &
  4 &
  4 &
  0.001 \\
 &
  m- &
  4 &
  6 &
  14 &
  14 &
  0.012 &
  13 &
  47 &
  0.025 &
  16 &
  53 &
  0.010 &
  6 &
  4 &
  1.051 &
  12 &
  15 &
  0.003 \\
 &
  m- &
  5 &
  10 &
  27 &
  26 &
  0.048 &
  27 &
  95 &
  0.015 &
  29 &
  105 &
  0.021 &
  31 &
  24 &
  46.885 &
  21 &
  23 &
  0.009 \\
 &
  m- &
  6 &
  20 &
  62 &
  60 &
  0.985 &
  62 &
  232 &
  0.036 &
  62 &
  276 &
  0.093 &
  64 &
  61 &
  0.015 &
  34 &
  27 &
  0.058 \\
 &
  m- &
  7 &
  35 &
  126 &
  96 &
  8.175 &
  126 &
  379 &
  0.066 &
  126 &
  475 &
  0.512 &
  128 &
  97 &
  0.031 &
  67 &
  65 &
  0.178 \\
\hline
avg &
   &
   &
   &
  47 &
  40 &
  1.844 &
  46 &
  153 &
  0.029 &
  47 &
  185 &
  0.128 &
  47 &
  38 &
  9.598 &
  \highlight{28} &
  27 &
  0.050 \\
\hline
\multirow{8}{*}{$\ket{D_n^k}$} &
  m- &
  3 &
  3 &
  4 &
  5 &
  0.002 &
  3 &
  18 &
  0.035 &
  6 &
  16 &
  0.004 &
  4 &
  3 &
  0.007 &
  4 &
  5 &
  0.001 \\
 &
  m- &
  4 &
  6 &
  14 &
  14 &
  0.011 &
  13 &
  47 &
  0.024 &
  16 &
  53 &
  0.009 &
  6 &
  4 &
  1.015 &
  12 &
  15 &
  0.003 \\
 &
  m- &
  5 &
  10 &
  27 &
  26 &
  0.051 &
  27 &
  95 &
  0.015 &
  29 &
  105 &
  0.022 &
  31 &
  24 &
  46.571 &
  21 &
  23 &
  0.010 \\
 &
  m- &
  6 &
  15 &
  50 &
  44 &
  0.263 &
  50 &
  167 &
  0.026 &
  48 &
  193 &
  0.051 &
  65 &
  62 &
  0.203 &
  44 &
  41 &
  0.026 \\
 &
  m- &
  7 &
  21 &
  76 &
  66 &
  1.447 &
  76 &
  255 &
  0.037 &
  72 &
  301 &
  0.254 &
  129 &
  129 &
  0.228 &
  70 &
  63 &
  0.051 \\
 &
  m- &
  8 &
  28 &
  107 &
  92 &
  7.766 &
  107 &
  359 &
  0.053 &
  107 &
  429 &
  1.384 &
  92 &
  76 &
  38.126 &
  101 &
  89 &
  0.098 \\
 &
  m- &
  9 &
  36 &
  143 &
  122 &
  51.022 &
  141 &
  477 &
  0.137 &
  147 &
  577 &
  6.208 &
  128 &
  106 &
  38.588 &
  137 &
  119 &
  0.194 \\
 &
  m- &
  10 &
  45 &
  184 &
  156 &
  309.848 &
  182 &
  609 &
  0.093 &
  186 &
  745 &
  30.987 &
  169 &
  140 &
  47.544 &
  178 &
  153 &
  0.423 \\
\hline
avg &
   &
   &
   &
  76 &
  66 &
  46.301 &
  75 &
  253 &
  0.052 &
  76 &
  302 &
  4.865 &
  78 &
  68 &
  21.535 &
  \highlight{71} &
  64 &
  0.101 \\
\hline
\multirow{6}{*}{$\ket{B_n^k}$} &
  n- &
  3 &
  3 &
  2 &
  3 &
  0.001 &
  2 &
  12 &
  0.005 &
  2 &
  15 &
  0.003 &
  2 &
  3 &
  0.002 &
  1 &
  3 &
  0.001 \\
 &
  n- &
  4 &
  7 &
  6 &
  7 &
  0.001 &
  6 &
  28 &
  0.007 &
  6 &
  35 &
  0.006 &
  6 &
  7 &
  0.179 &
  5 &
  7 &
  0.002 \\
 &
  n- &
  5 &
  15 &
  14 &
  15 &
  0.002 &
  14 &
  60 &
  0.011 &
  14 &
  75 &
  0.012 &
  16 &
  18 &
  0.246 &
  13 &
  15 &
  0.007 \\
 &
  n- &
  6 &
  31 &
  30 &
  31 &
  0.004 &
  30 &
  124 &
  0.080 &
  30 &
  155 &
  0.050 &
  32 &
  34 &
  0.252 &
  29 &
  31 &
  0.027 \\
 &
  n- &
  7 &
  63 &
  62 &
  63 &
  0.007 &
  62 &
  252 &
  0.050 &
  62 &
  315 &
  0.269 &
  64 &
  66 &
  0.288 &
  61 &
  63 &
  0.097 \\
 &
  n- &
  8 &
  127 &
  126 &
  127 &
  0.017 &
  126 &
  508 &
  0.209 &
  126 &
  635 &
  1.769 &
  128 &
  130 &
  0.321 &
  125 &
  127 &
  0.380 \\
\hline
avg &
   &
   &
   &
  40 &
  41 &
  0.005 &
  40 &
  164 &
  0.060 &
  40 &
  205 &
  0.352 &
  41 &
  43 &
  0.215 &
  \highlight{39} &
  41 &
  0.086 \\
\hline
\multirow{5}{*}{$\ket{B_n^k}$} &
  n- &
  3 &
  5 &
  6 &
  6 &
  0.001 &
  6 &
  23 &
  0.007 &
  6 &
  25 &
  0.005 &
  4 &
  5 &
  0.095 &
  2 &
  5 &
  0.001 \\
 &
  n- &
  4 &
  9 &
  14 &
  14 &
  0.002 &
  14 &
  55 &
  0.009 &
  14 &
  65 &
  0.010 &
  6 &
  7 &
  4.556 &
  3 &
  7 &
  0.004 \\
 &
  n- &
  5 &
  17 &
  30 &
  30 &
  0.003 &
  30 &
  119 &
  0.017 &
  30 &
  145 &
  0.024 &
  22 &
  23 &
  4.618 &
  4 &
  9 &
  0.012 \\
 &
  n- &
  6 &
  33 &
  62 &
  62 &
  0.005 &
  62 &
  247 &
  0.033 &
  62 &
  305 &
  0.070 &
  54 &
  55 &
  4.547 &
  5 &
  11 &
  0.042 \\
 &
  n- &
  7 &
  65 &
  126 &
  126 &
  0.011 &
  126 &
  503 &
  0.070 &
  126 &
  625 &
  0.675 &
  118 &
  119 &
  4.570 &
  6 &
  13 &
  0.152 \\
\hline
avg &
   &
   &
   &
  48 &
  48 &
  0.004 &
  48 &
  189 &
  0.027 &
  48 &
  233 &
  0.157 &
  41 &
  42 &
  3.677 &
  \highlight{4} &
  9 &
  0.042 \\
\hline
\multirow{5}{*}{URand.} &
  n- &
  3 &
  4 &
  6 &
  7 &
  0.001 &
  6 &
  28 &
  0.006 &
  6 &
  35 &
  0.006 &
  4 &
  6 &
  0.077 &
  3 &
  6 &
  0.001 \\
 &
  n- &
  4 &
  8 &
  14 &
  15 &
  0.001 &
  14 &
  59 &
  0.010 &
  14 &
  75 &
  0.011 &
  9 &
  10 &
  32.952 &
  13 &
  15 &
  0.005 \\
 &
  n- &
  5 &
  16 &
  30 &
  31 &
  0.003 &
  30 &
  124 &
  0.019 &
  30 &
  155 &
  0.093 &
  33 &
  33 &
  0.181 &
  29 &
  31 &
  0.018 \\
 &
  n- &
  6 &
  32 &
  62 &
  56 &
  0.005 &
  62 &
  224 &
  0.033 &
  62 &
  280 &
  0.089 &
  64 &
  58 &
  0.015 &
  61 &
  56 &
  0.063 \\
 &
  n- &
  7 &
  64 &
  126 &
  121 &
  0.009 &
  126 &
  484 &
  0.074 &
  126 &
  605 &
  0.541 &
  128 &
  123 &
  0.038 &
  125 &
  121 &
  0.260 \\
\hline
avg &
   &
   &
   &
  48 &
  46 &
  0.004 &
  48 &
  184 &
  0.028 &
  48 &
  230 &
  0.148 &
  48 &
  46 &
  6.653 &
  \highlight{46} &
  46 &
  0.070 \\
\hline
\multirow{5}{*}{Rand.} &
  n- &
  3 &
  4 &
  6 &
  7 &
  0.001 &
  6 &
  28 &
  0.007 &
  6 &
  35 &
  0.005 &
  5 &
  5 &
  0.083 &
  3 &
  5 &
  0.001 \\
 &
  n- &
  4 &
  8 &
  14 &
  15 &
  0.001 &
  14 &
  60 &
  0.010 &
  14 &
  75 &
  0.011 &
  16 &
  17 &
  73.198 &
  11 &
  14 &
  0.005 \\
 &
  n- &
  5 &
  16 &
  30 &
  31 &
  0.002 &
  30 &
  124 &
  0.019 &
  30 &
  155 &
  0.027 &
  33 &
  33 &
  0.204 &
  29 &
  31 &
  0.017 \\
 &
  n- &
  6 &
  32 &
  62 &
  63 &
  0.004 &
  62 &
  252 &
  0.044 &
  62 &
  315 &
  0.097 &
  64 &
  65 &
  0.016 &
  61 &
  63 &
  0.061 \\
 &
  n- &
  7 &
  64 &
  126 &
  127 &
  0.010 &
  126 &
  508 &
  0.088 &
  126 &
  635 &
  0.721 &
  128 &
  129 &
  0.038 &
  125 &
  127 &
  0.304 \\
\hline
avg &
   &
   &
   &
  48 &
  49 &
  0.004 &
  48 &
  194 &
  0.033 &
  48 &
  243 &
  0.172 &
  49 &
  50 &
  14.708 &
  \highlight{46} &
  48 &
  0.077 \\
\hline
\multirow{9}{*}{URand.} &
  n- &
  3 &
  3 &
  4 &
  5 &
  0.001 &
  3 &
  21 &
  0.014 &
  3 &
  20 &
  0.004 &
  3 &
  3 &
  0.003 &
  2 &
  3 &
  0.001 \\
 &
  n- &
  4 &
  4 &
  10 &
  8 &
  0.001 &
  9 &
  30 &
  0.015 &
  9 &
  32 &
  0.007 &
  3 &
  2 &
  0.003 &
  9 &
  6 &
  0.003 \\
 &
  m- &
  5 &
  5 &
  10 &
  10 &
  0.009 &
  9 &
  35 &
  0.037 &
  12 &
  36 &
  0.008 &
  10 &
  7 &
  1.502 &
  10 &
  10 &
  0.003 \\
 &
  m- &
  6 &
  6 &
  17 &
  13 &
  0.027 &
  16 &
  46 &
  0.040 &
  21 &
  46 &
  0.015 &
  15 &
  10 &
  1.491 &
  17 &
  13 &
  0.004 \\
 &
  m- &
  7 &
  7 &
  23 &
  18 &
  0.054 &
  22 &
  63 &
  0.040 &
  27 &
  66 &
  0.098 &
  20 &
  14 &
  27.088 &
  21 &
  19 &
  0.009 \\
 &
  m- &
  8 &
  8 &
  25 &
  19 &
  0.153 &
  24 &
  62 &
  0.039 &
  27 &
  67 &
  0.388 &
  24 &
  17 &
  6.372 &
  23 &
  20 &
  0.035 \\
 &
  m- &
  9 &
  9 &
  32 &
  22 &
  0.879 &
  30 &
  76 &
  0.025 &
  34 &
  85 &
  1.390 &
  32 &
  19 &
  1.491 &
  32 &
  22 &
  0.019 \\
 &
  m- &
  10 &
  10 &
  44 &
  25 &
  1.109 &
  39 &
  102 &
  0.064 &
  48 &
  106 &
  6.521 &
  40 &
  22 &
  0.098 &
  41 &
  26 &
  0.013 \\
 &
  m- &
  11 &
  11 &
  56 &
  28 &
  6.333 &
  55 &
  104 &
  0.042 &
  60 &
  117 &
  32.147 &
  56 &
  25 &
  0.044 &
  56 &
  28 &
  0.027 \\
\hline
avg &
   &
   &
   &
  25 &
  16 &
  1.0 &
  23 &
  60 &
  0.0 &
  27 &
  64 &
  4.5 &
  23 &
  13 &
  4.2 &
  23 &
  16 &
  0.0 \\
\hline
\multirow{9}{*}{Rand.} &
  n- &
  3 &
  3 &
  4 &
  5 &
  0.001 &
  3 &
  21 &
  0.013 &
  3 &
  17 &
  0.004 &
  3 &
  3 &
  0.003 &
  2 &
  3 &
  0.001 \\
 &
  n- &
  4 &
  4 &
  14 &
  15 &
  0.001 &
  14 &
  60 &
  0.010 &
  14 &
  76 &
  0.011 &
  5 &
  6 &
  0.077 &
  10 &
  11 &
  0.003 \\
 &
  m- &
  5 &
  5 &
  11 &
  8 &
  0.008 &
  10 &
  28 &
  0.024 &
  13 &
  35 &
  0.008 &
  10 &
  7 &
  0.083 &
  10 &
  8 &
  0.002 \\
 &
  m- &
  6 &
  6 &
  18 &
  14 &
  0.024 &
  18 &
  39 &
  0.010 &
  22 &
  45 &
  0.016 &
  16 &
  11 &
  1.087 &
  17 &
  15 &
  0.007 \\
 &
  m- &
  7 &
  7 &
  19 &
  14 &
  0.021 &
  18 &
  50 &
  0.027 &
  21 &
  55 &
  0.098 &
  17 &
  13 &
  7.409 &
  16 &
  15 &
  0.006 \\
 &
  m- &
  8 &
  8 &
  28 &
  16 &
  0.160 &
  26 &
  61 &
  0.020 &
  32 &
  66 &
  0.349 &
  28 &
  13 &
  1.578 &
  28 &
  16 &
  0.007 \\
 &
  m- &
  9 &
  9 &
  36 &
  24 &
  0.492 &
  33 &
  83 &
  0.046 &
  42 &
  84 &
  1.262 &
  35 &
  20 &
  0.112 &
  35 &
  25 &
  0.029 \\
 &
  m- &
  10 &
  10 &
  46 &
  25 &
  2.199 &
  46 &
  86 &
  0.020 &
  50 &
  94 &
  6.347 &
  44 &
  22 &
  1.536 &
  46 &
  25 &
  0.054 \\
 &
  m- &
  11 &
  11 &
  56 &
  28 &
  4.217 &
  56 &
  95 &
  0.024 &
  60 &
  106 &
  32.971 &
  51 &
  25 &
  0.034 &
  56 &
  28 &
  0.096 \\
\hline
avg &
   &
   &
   &
  26 &
  17 &
  0.791 &
  25 &
  58 &
  0.021 &
  29 &
  64 &
  4.563 &
  \highlight{23} &
  13 &
  1.324 &
  24 &
  16 &
  0.023 \\
\hline
Avg. &
   &
   &
   &
  42 &
  37 &
  7.192 &
  41 &
  142 &
  0.039 &
  43 &
  171 &
  2.305 &
  41 &
  35 &
  7.267 &
  34 &
  31 &
  0.052 \\
Impr &
   &
   &
   &
   &
   &
   &
  1.66\% &
   &
  0.55\% &
  -3.20\% &
   &
  32.05\% &
  1.75\% &
   &
  101\% &
  \highlight{17.29\%} &
   &
  0.72\% \\
\hline
\end{tabular}
\caption{Experimental results. ``\#G2'' and ``\#G'' represents the number of two-qubit and single-qubit gates. \todo{figure out why PyZX (GA) gets even worse results.}}
\label{tab:results}
\end{table*}
